Pushdown Abstractions of JavaScript

We design a family of program analyses for JavaScript that make no approximation in matching calls with returns, exceptions with handlers, and breaks with labels. We do so by starting from an established reduction semantics for JavaScript and systematically deriving its intensional abstract interpretation. Our first step is to transform the semantics into an equivalent low-level abstract machine: the JavaScript Abstract Machine (JAM). We then give an infinite-state yet decidable pushdown machine whose stack precisely models the structure of the concrete program stack. The precise model of stack structure in turn confers precise control-flow analysis even in the presence of control effects, such as exceptions and finally blocks. We give pushdown generalizations of traditional forms of analysis such as k-CFA, and prove the pushdown framework for abstract interpretation is sound and computable.

==> local-macros.tex <==
\makeatletter
\newbox\xrat@above
\newcommand{\xmultistepsto}[1][]{%
  \setbox\xrat@above=\hbox{\ensuremath{\scriptstyle #1}}%
  \pgfmathsetlengthmacro{\xrat@len}{max(\wd\xrat@above,1em)+1em}%
  \mathrel{\tikz [|->>,baseline=-.75ex]
                 \draw (0,0) -- node[below=-2pt] {}
                                node[above=-2pt] {\box\xrat@above}
                       (\xrat@len,0) ;}}
\makeatother

\makeatletter
\newbox\xrat@above
\newcommand{\xstepsto}[1][]{%
  \setbox\xrat@above=\hbox{\ensuremath{\scriptstyle #1}}%
  \pgfmathsetlengthmacro{\xrat@len}{max(\wd\xrat@above,.5em)+1em}%
  \;\mathrel{\tikz [|->,baseline=-.75ex]
                 \draw (0,0) -- node[below=-2pt] {}
                                node[above=-2pt] {\box\xrat@above}
                       (\xrat@len,0) ;}\;}
\makeatother


\newcommand\jscode{\sffamily\bfseries}
\renewcommand{\ttlp}{\mbox{\tt (}}
\renewcommand{\ttrp}{\mbox{\tt )}}
\newcommand{\ttlb}{\mbox{\tt [}}
\newcommand{\ttrb}{\mbox{\tt ]}}
\renewcommand{\ttlc}{\mbox{\tt\{}}
\renewcommand{\ttrc}{\mbox{\tt\}}}
\newcommand{\tteq}{\mbox{\tt=}}

\renewcommand\vec[1]{\overline{#1}}

% \newtheorem{theorem}{Theorem}

\newcommand{\evalf}{\mathit{eval}}
\newcommand{\avalf}{\mathit{aval}}

% Machine names
\newcommand{\CESK}{{\mathit{CESK}}}
\newcommand{\ACESK}{{\widehat{\mathit{CSK}}}}

\newcommand{\multistep}{\longmapsto\!\!\!\!\!\rightarrow}


\newcommand{\aDelta}{\widehat{\Delta}}
\newcommand{\aConf}{\sa{Conf}}

\newcommand{\p}{_+}
\newcommand{\m}{_-}
\newcommand{\pam}{_\pm}


%% \newcommand{\conf}{\var{c}}
%% \newcommand{\state}{\varsigma}
%% \newcommand{\env}{\rho}
%% \newcommand{\store}{\sigma}

\newcommand\getf[2]{\mathit{get}({#1},{#2})}
\newcommand\putf[3]{\mathit{put}({#1},{#2},{#3})}
\newcommand\allocf[1]{\mathit{alloc}({#1})}

\newcommand\getff{\mathit{get}}
\newcommand\putff{\mathit{put}}
\newcommand\allocff{\mathit{alloc}}

\newcommand\agetff{\widehat{\getff}}
\newcommand\aputff{\widehat{\putff}}
\newcommand\aallocff{\widehat{\allocff}}
\newcommand\agetf[2]{\agetff({#1},{#2})}
\newcommand\aputf[3]{\aputff({#1},{#2},{#3})}
\newcommand\aallocf[1]{\aallocff({#1})}

%% \newcommand\agetf[2]{\widehat{\mathit{get}}({#1},{#2})}
%% \newcommand\aputf[3]{\widehat{\mathit{put}}({#1},{#2},{#3})}
%% \newcommand\aallocf[1]{\widehat{\mathit{alloc}}({#1})}

\newcommand\inj{\mathit{inj}}
\newcommand\JAM{\mathit{JAM}}
\newcommand\JAMP{\mathit{JAM}^*}
\newcommand\AJAMP{\widehat{\mathit{JAM^*}}}
\newcommand\AJAM{\widehat{\mathit{JAM}}}

\newcommand\AJAMPRIME{\widehat{\mathit{JAM}}\;\!'}

\newcommand\kfar[3]{\mathbf{c_2}({#1},{#2},{#3})}
\newcommand\kffn[2]{\mathbf{c_3}({#1},{#2})}

\newcommand\xptr{\mathbf{x}(a)}
\newcommand\cptr{\mathbf{c}(a)}
\newcommand\dptr{\mathbf{d}(a)}


% \newcommand{\Den}{Val} % Denotable values
%% \newcommand{\vv}{x}
%% \newcommand{\expr}{e}
%% \newcommand{\ttlp}{\mbox{\tt (}}
%% \newcommand{\ttrp}{\mbox{\tt )}}
%% \newcommand{\appform}[2]{\ttlp #1\; #2\ttrp}
%% \newcommand\numeral[1]{\ulcorner{#1}\urcorner}
\newcommand\mtk{\mathbf{mt}}
\newcommand\fnk{\mathbf{fn}}
\newcommand\ark{\mathbf{ar}}
\newcommand\mte{\varnothing} % mt env
\newcommand\mts{\varnothing} % mt store
%% \newcommand{\den}{v}
%% \newcommand{\aden}{v}
%% \newcommand{\addr}{a}
%% \newcommand{\aaddr}{\hat{a}}
%% \newcommand{\dom}{\var{dom}}


%% FJ stuff
%% \newcommand{\mclassdef}{L}
%% \newcommand{\mconsdef}{K}
%% \newcommand{\mmethdef}{M}
%% \newcommand{\mmethdefs}{\vec\mmethdef}
%% \newcommand{\mmeth}{m}
%% \newcommand{\mclass}{C}
%% \newcommand{\mclasso}{D}
%% \newcommand{\mclasss}{\vec\mclass}
\newcommand{\mexp}{e}
\newcommand{\mexpo}{f}
\newcommand{\mexpoo}{g} % ha ha
\newcommand{\mval}{v}
\newcommand{\mvalo}{u}
\newcommand{\mvaloo}{t}
%% \newcommand{\mvalo}{u}
\newcommand{\mvals}{\vec\mval}
%% \newcommand{\mvalso}{\vec\mvalo}
\newcommand{\mexps}{\vec\mexp}
\newcommand{\mexpso}{\vec\mexpo}
\newcommand{\mvar}{x}
\newcommand{\mvars}{\vec\mvar}
%% \newcommand{\mfld}{f}
%% \newcommand{\mflds}{\vec\mfld}
\newcommand{\sdot}[2]{{#1}\ttdot{#2}}
%% \newcommand{\sinv}[3]{{#1}\ttdot{#2}\ttlp{#3}\ttrp}
%% \newcommand{\snew}[2]{{\text{\tt new}}\;{#1}\ttlp{#2}\ttrp}
%% \newcommand{\scast}[2]{\ttlp{#1}\ttrp{#2}}
%% \newcommand{\sthis}{\text{\tt this}}
%% \newcommand{\sreturn}{\text{\tt return}}
\newcommand{\mctx}{\mathcal{E}}
\newcommand{\mcctx}{\mathcal{C}}
\newcommand{\mdctx}{\mathcal{D}}
\newcommand{\mectx}{\mathcal{E}}
\newcommand{\mfctx}{\mathcal{F}}
\newcommand{\mgctx}{\mathcal{G}}
\newcommand{\mhctx}{\mathcal{H}}

\newcommand{\msctx}{\mathcal{S}}

%% \newcommand{\fieldsf}{\mathit{fields}}
%% \newcommand{\mbodyf}{\mathit{mbody}}
%% \newcommand{\subtypef}[2]{{#1}<:{#2}}
\newcommand{\stepsto}{\rightarrow}
\newcommand{\multistepsto}{\rightarrow^*}

\newcommand{\scls}[2]{({#1},{#2})}
\newcommand{\mcls}{c}
\newcommand{\mclso}{d}
\newcommand{\mclss}{\vec{c}}

\newcommand{\mtenv}{\varnothing} %\mathbf{nil}}
\newcommand{\mtsto}{\varnothing} %\mathbf{nil}}

\newcommand{\mhole}{\bullet}%[\;]}

\newcommand{\mans}{A}

\newcommand{\crangle}{\rangle_{\mathit{co}}}
\newcommand{\erangle}{\rangle_{\mathit{ev}}}
\newcommand{\arangle}{\rangle_{\mathit{ap}}}
\newcommand{\mCTX}{C}
\newcommand{\mDTX}{D}
\newcommand{\mETX}{E}
\newcommand{\CTX}[1]{\mathbf{C}_{#1}}
\newcommand{\DTX}[1]{\mathbf{D}_{#1}}
\newcommand{\ETX}[1]{\mathbf{E}_{#1}}
\newcommand{\mtseq}{\epsilon}

\newcommand{\cons}[2]{{#1}::{#2}}
\newcommand{\nil}{\mathbf{nil}}

\newcommand{\UNLD}{\mathcal{U}}
\newcommand{\mclos}{c}
\newcommand{\mcloss}{\vec\mclos}
\newcommand{\menv}{\rho}
\newcommand{\msto}{\sigma}
\newcommand{\masto}{\hat\msto}
\newcommand{\maddr}{a}
\newcommand{\maddrs}{\vec\maddr}
\newcommand{\mkont}{C} % \kappa
\newcommand{\kmt}{\mathbf{c_1}}
\newcommand{\kfld}[2]{\mathbf{c_2}({#1},{#2})}
\newcommand{\kinv}[4]{\mathbf{c_3}({#1},{#2},{#3},{#4})}
\newcommand{\karg}[5]{\mathbf{c_4}({#1},{#2},{#3},{#4},{#5})}
\newcommand{\knew}[5]{\mathbf{c_5}({#1},{#2},{#3},{#4},{#5})}
\newcommand{\kcas}[2]{\mathbf{c_6}({#1},{#2})}


\newcommand\mlab{{\lab}}



\newcommand{\semi}{\mbox{\tt;}}
\newcommand{\ttcol}{\mbox{\tt:}}
\newcommand{\ttdot}{\mbox{\tt.}}
\newcommand{\snull}{\text{\jscode{null}}}
\newcommand{\sundefn}{\text{\jscode{undef}}}
\newcommand{\mconst}{k}
\newcommand{\sfunc}[2]{\text{\jscode fun}\ttlp{#1}\ttrp\;\ttlc\;{#2}\;\ttrc}
\newcommand{\srec}[1]{\ttlc{#1}\ttrc}
% \newcommand{\mconst}{\mathit{k}}
\newcommand{\mstr}{\mathit{s}}
\newcommand{\mbool}{\mathit{b}}
\newcommand{\mnum}{\mathit{n}}
\newcommand{\scol}[2]{{#1}\-\ttcol\-{#2}}
\newcommand{\strue}{\text{\jscode true}}
\newcommand{\sfalse}{\text{\jscode false}}
\newcommand{\slet}[3]{\text{\jscode let}\;\ttlp{#1}\;\tteq\;{#2}\ttrp\;{#3}}
\newcommand{\sapp}[2]{{#1}\ttlp{#2}\ttrp}
\newcommand{\saref}[2]{{#1}\ttlb{#2}\ttrb}
\newcommand{\saset}[3]{\saref{#1}{#2}\;\tteq\;{#3}}
\newcommand{\sdel}[2]{\text{\jscode del}\;\saref{#1}{#2}}
\newcommand{\sset}[2]{{#1}\;\tteq\;{#2}}
\newcommand{\sref}[1]{\text{\jscode ref}\;{#1}}
\newcommand{\sderef}[1]{\text{\jscode deref}\;{#1}}
%\newcommand{\sif}[3]{\text{\jscode if}\;\ttlp{#1}\ttrp\;\ttlc\;{#2}\;\ttrc\;\text{\jscode else}\;\ttlc\;{#3}\;\ttrc}
\newcommand{\sif}[3]{\text{\jscode if}\ttlp{#1}\ttrp\ttlc{#2}\ttrc\ttlc{#3}\ttrc}
\newcommand{\sseq}[2]{{#1}\semi{#2}}
\newcommand{\swhile}[2]{\text{\jscode while}\ttlp{#1}\ttrp\ttlc{#2}\ttrc}
\newcommand{\slab}[2]{{\scol{#1}{\ttlc\;{#2}\;\ttrc}}}
\newcommand{\sbreak}[2]{\text{\jscode break}\;{#1}\;{#2}}
\newcommand{\stryc}[3]{\text{\jscode try}\;\ttlc{#1}\ttrc\;\text{\jscode catch}\;\ttlp{#2}\ttrp\ttlc{#3}\ttrc}
\newcommand{\stryf}[2]{\text{\jscode try}\;\ttlc{#1}\ttrc\;\text{\jscode finally}\;\ttlc{#2}\ttrc}
\newcommand{\sthrow}[1]{\text{\jscode throw}\;{#1}}
\newcommand{\serr}[1]{\text{\jscode err}\;{#1}}
\newcommand{\sop}[1]{\mathit{op}\ttlp{#1}\ttrp}
\newcommand{\sopn}[1]{\mathit{op_n}\ttlp{#1}\ttrp}

\newcommand{\mop}{\mathit{op}}

\newcommand{\splus}[1]{\text{\jscode plus}\ttlp#1\ttrp}

\newcommand{\mmap}{p}
%\newcommand{\mmapv}{q}
\newcommand{\mmapc}{q}
\newcommand{\mmaps}{\vec\mmap}
%\newcommand{\mmapvs}{\vec\mmapv}
\newcommand{\mmapcs}{\vec\mmapc}

\newcommand{\klet}[4]{\mathbf{c_2}({#1},{#2},{#3},{#4})}       % let
\newcommand{\kar}[3]{\mathbf{c_3}({#1},{#2},{#3})}              % ar
\newcommand{\kfn}[5]{\mathbf{c_4}({#1},{#2},{#3},{#4},{#5})}    % fn
\newcommand{\krec}[5]{\mathbf{c_5}({#1},{#2},{#3},{#4},{#5})}  % rec
\newcommand{\kind}[3]{\mathbf{c_6}({#1},{#2},{#3})}            % ind
\newcommand{\kref}[2]{\mathbf{c_7}({#1},{#2})}                 % ref
\newcommand{\kindb}[4]{\mathbf{c_8}({#1},{#2},{#3},{#4})}     % uind
\newcommand{\krefb}[4]{\mathbf{c_9}({#1},{#2},{#3},{#4})}     % uref
\newcommand{\ksetb}[3]{\mathbf{c_{10}}({#1},{#2},{#3})}          % uset
\newcommand{\kindd}[3]{\mathbf{c_{11}}({#1},{#2},{#3})}          % dind
\newcommand{\krefd}[2]{\mathbf{c_{12}}({#1},{#2})}               % dref

